The Ages of M31 Star Clusters: Spectral Energy Distribution Versus Color-Magnitude Diagram

It is well-known that fitting the Color Magnitude Diagrams (CMDs) to the theoretical isochrones is the main method to determine star cluster ages. However, when the CMDs are not available, the Spectral Energy Distribution (SED)-fitting technique is the only other approach, although it suffers the age-metallicity-reddening degeneracy. In this work, we gather the ages, metallicities and masses of dozens of M31 star clusters from the CMD-fitting with HST images from the literatures for comparison. We check the reliability of the SED-fitting results with different models, i.e., Bruzual \& Charlot 2003 model (BC03), Galaxy Evolutionary Synthesis Models ({\sl GALEV}) and Advanced Stellar Population Synthesis (ASPS) for the simple stellar populations (SSPs) with single stars (ss)-SSP/binary star (bs)-SSPs models. The photometry bands includes the Galaxy Evolution Explorer {\sl GALEX} FUV/NUV bands, optical/near-infrared $UBVRIJHK$ bands, as well as the Wide-field Infrared Survey Explorer ({\sl WISE}) $W1$/$W2$ bands. The comparisons show that the SED-fitting ages agree well with the CMD-fitting ages, either with the fixed metallicity or with the free metallicity for both the BC03 and the {\sl GALEV} model. However, for the ASPS models, it seems that SED-fitting results are systematic older than the CMD ages, especially for the ages log t <9.0 (yr). The fitting also shows that the {\sl GALEX} FUV/NUV-band are more important than the {\sl WISE} $W1$/$W2$ for constraining the ages, which confirms the previous findings. We also derived the masses of our sample star clusters from the BC03 and {\sl GALEV} models and it is found that the values agree well with that in the literature.

==> krosed_GALEV_result_cmd.tex <==
   B015D-D041 & $   -0.35_{ -1.06}^{+  0.12} $ &  -0.02 &  $    8.03_{ -0.07}^{+  0.03} $ & $    7.85_{ -0.15}^{+  0.15} $ & $  4.05_{ -0.05}^{+  0.04} $ &  4.20 \\
    B040-G102 & $   -0.35_{ -0.72}^{+  0.21} $ &  -0.02 &  $    8.00_{ -0.16}^{+  0.07} $ & $    7.90_{ -0.15}^{+  0.20} $ & $  4.07_{ -0.08}^{+  0.08} $ &  4.60 \\
    B043-G106 & $   -0.38_{ -0.92}^{+  0.16} $ &  -0.02 &  $    7.96_{ -0.20}^{+  0.06} $ & $    7.90_{ -0.15}^{+  0.20} $ & $  4.20_{ -0.11}^{+  0.05} $ &  4.40 \\
    B066-G128 & $    0.40_{ -1.25}^{+  0.00} $ &  -0.02 &  $    7.45_{ -0.34}^{+  0.30} $ & $    7.85_{ -0.15}^{+  0.15} $ & $  3.73_{ -0.38}^{+  0.14} $ &  4.20 \\
    B081-G142 & $   -1.38_{ -0.32}^{+  0.66} $ &  -0.02 &  $    8.70_{ -0.35}^{+  0.21} $ & $    8.15_{ -0.15}^{+  0.15} $ & $  4.59_{ -0.28}^{+  0.18} $ &  5.10 \\
   B257D-D073 & $   -0.10_{ -1.07}^{+  0.50} $ &  -0.02 &  $    8.06_{ -0.22}^{+  0.32} $ & $    7.90_{ -0.15}^{+  0.20} $ & $  4.15_{ -0.16}^{+  0.25} $ &  4.60 \\
    B318-G042 & $   -0.42_{ -0.85}^{+  0.32} $ &  -0.40 &  $    7.86_{ -0.28}^{+  0.13} $ & $    7.85_{ -0.15}^{+  0.15} $ & $  4.06_{ -0.15}^{+  0.10} $ &  3.80 \\
    B321-G046 & $   -0.31_{ -0.56}^{+  0.22} $ &   0.65 &  $    8.06_{ -0.04}^{+  0.07} $ & $    8.23_{ -0.15}^{+  0.10} $ & $  4.01_{ -0.06}^{+  0.08} $ &  4.20 \\
    B327-G053 & $   -0.38_{ -0.69}^{+  0.38} $ &  -0.40 &  $    7.68_{ -0.24}^{+  0.26} $ & $    7.70_{ -0.10}^{+  0.15} $ & $  4.21_{ -0.12}^{+  0.21} $ &  4.50 \\
    B376-G309 & $   -0.38_{ -0.97}^{+  0.78} $ &  -0.02 &  $    8.00_{ -0.20}^{+  0.17} $ & $    8.00_{ -0.15}^{+  0.15} $ & $  3.86_{ -0.09}^{+  0.22} $ &  4.10 \\
    B448-D035 & $    0.40_{ -0.75}^{+  0.00} $ &  -0.02 &  $    8.29_{ -0.20}^{+  0.08} $ & $    7.90_{ -0.15}^{+  0.20} $ & $  4.44_{ -0.22}^{+  0.04} $ &  4.10 \\
    B475-V128 & $   -1.70_{  0.00}^{+  0.54} $ &  -0.40 &  $    8.70_{ -0.68}^{+  0.30} $ & $    8.30_{ -0.20}^{+  0.20} $ & $  4.57_{ -0.31}^{+  0.20} $ &  4.70 \\
         V031 & $    0.40_{ -1.33}^{+  0.00} $ &  -0.70 &  $    8.20_{ -0.33}^{+  0.38} $ & $    8.45_{ -0.15}^{+  0.15} $ & $  4.13_{ -0.30}^{+  0.24} $ &  4.80 \\
   VDB0-B195D & $   -0.38_{ -0.51}^{+  0.04} $ &  -0.02 &  $    7.92_{ -0.19}^{+  0.07} $ & $    7.40_{ -0.30}^{+  0.30} $ & $  5.01_{ -0.14}^{+  0.03} $ & 99.99 \\
    B083-G146 & $   -1.70_{  0.00}^{+  0.26} $ &  -0.40 &  $    9.30_{ -0.07}^{+  0.16} $ & $    8.70_{  0.00}^{+  1.44} $ & $  4.76_{ -0.03}^{+  0.14} $ &  4.70 \\
    B222-G277 & $   -0.31_{ -0.14}^{+  0.15} $ &  -0.02 &  $    8.96_{ -0.04}^{+  0.04} $ & $    8.60_{  0.00}^{+  1.54} $ & $  4.59_{ -0.04}^{+  0.05} $ &  4.60 \\
    B347-G154 & $   -1.63_{ -0.07}^{+  0.27} $ &  -0.40 &  $    9.46_{ -0.07}^{+  0.08} $ & $    8.80_{  0.00}^{+  1.34} $ & $  4.96_{ -0.06}^{+  0.07} $ &  4.70 \\
    B374-G306 & $   -0.06_{ -0.54}^{+  0.46} $ &  -0.02 &  $    8.40_{ -0.26}^{+  0.18} $ & $    8.50_{  0.00}^{+  1.64} $ & $  4.05_{ -0.23}^{+  0.19} $ &  3.90 \\
         NB16 & $    0.08_{ -0.50}^{+  0.19} $ &  -0.02 &  $    9.24_{ -0.24}^{+  0.32} $ & $    8.70_{  0.00}^{+  1.44} $ & $  4.94_{ -0.34}^{+  0.32} $ &  4.80 \\
    B049-G112 & $   -0.42_{ -1.27}^{+  0.35} $ &  -0.02 &  $    8.70_{ -0.27}^{+  0.16} $ & $    8.45_{ -0.20}^{+  0.20} $ & $  4.48_{ -0.34}^{+  0.17} $ &  4.50 \\
    B367-G292 & $    0.40_{ -0.11}^{+  0.00} $ &  -0.02 &  $    8.19_{ -0.03}^{+  0.06} $ & $    8.30_{ -0.20}^{+  0.20} $ & $  4.03_{ -0.04}^{+  0.03} $ &  4.30 \\
    B458-D049 & $    0.01_{ -0.15}^{+  0.24} $ &  -0.02 &  $    8.50_{ -0.12}^{+  0.15} $ & $    8.50_{ -0.20}^{+  0.20} $ & $  4.23_{ -0.08}^{+  0.15} $ &  4.10 \\
  B521-SK034A & $   -0.38_{ -0.57}^{+  0.05} $ &  -0.02 &  $    7.96_{ -0.05}^{+  0.04} $ & $    8.60_{ -0.30}^{+  0.30} $ & $  3.76_{ -0.02}^{+  0.02} $ &  3.90 \\
         M039 & $   -0.21_{ -1.49}^{+  0.60} $ &  -0.02 &  $    8.34_{ -0.69}^{+  0.40} $ & $    8.50_{ -0.20}^{+  0.20} $ & $  3.50_{ -0.37}^{+  0.36} $ &  3.80 \\
         M050 & $    0.40_{ -0.33}^{+  0.00} $ &  -0.02 &  $    7.90_{ -0.13}^{+  0.36} $ & $    8.75_{ -0.30}^{+  0.30} $ & $  3.49_{ -0.13}^{+  0.20} $ &  4.30 \\
    B315-G038 & $   -1.41_{ -0.28}^{+  0.57} $ &  -0.40 &  $    8.00_{ -0.18}^{+  0.02} $ & $    8.00_{ -0.20}^{+  0.15} $ & $  4.67_{ -0.11}^{+  0.00} $ &  4.60 \\
    B319-G044 & $   -1.56_{ -0.14}^{+  0.83} $ &  -0.40 &  $    8.00_{ -0.29}^{+  0.04} $ & $    8.00_{ -0.20}^{+  0.15} $ & $  4.07_{ -0.20}^{+ -0.02} $ &  3.90 \\
    B342-G094 & $   -0.38_{ -0.96}^{+  0.72} $ &  -0.40 &  $    8.00_{ -0.16}^{+  0.08} $ & $    8.20_{ -0.20}^{+  0.15} $ & $  3.87_{ -0.07}^{+  0.16} $ &  4.00 \\
    B368-G293 & $    0.40_{ -0.48}^{+  0.00} $ &  -0.02 &  $    7.30_{ -0.27}^{+  0.45} $ & $    7.80_{ -0.10}^{+  0.10} $ & $  3.57_{ -0.43}^{+  0.22} $ &  4.40 \\
    B292-G010 & $   -1.70_{  0.00}^{+  0.23} $ &  -1.82 &  $    9.24_{ -0.12}^{+  0.06} $ & $    9.80_{  0.00}^{+  0.34} $ & $  4.62_{ -0.12}^{+  0.04} $ & 99.99 \\
    B337-G068 & $   -1.09_{ -0.20}^{+  0.13} $ &  -1.30 &  $    9.27_{ -0.07}^{+  0.07} $ & $    9.65_{  0.00}^{+  0.49} $ & $  4.78_{ -0.05}^{+  0.06} $ & 99.99 \\
    B350-G162 & $   -1.63_{ -0.07}^{+  0.20} $ &  -1.52 &  $    9.31_{ -0.04}^{+  0.08} $ & $    9.75_{  0.00}^{+  0.39} $ & $  4.79_{ -0.02}^{+  0.08} $ & 99.99 \\


==> krosed_GALEV_result_cmd_fixz.tex <==
   B015D-D041 &   -0.02 &  $    7.83_{ -0.28}^{+  0.05} $ & $    7.85_{ -0.15}^{+  0.15} $ & $  3.99_{ -0.15}^{+  0.03} $ &  4.20 \\
    B040-G102 &   -0.02 &  $    7.81_{ -0.21}^{+  0.27} $ & $    7.90_{ -0.15}^{+  0.20} $ & $  4.01_{ -0.12}^{+  0.16} $ &  4.60 \\
    B043-G106 &   -0.02 &  $    7.81_{ -0.22}^{+  0.09} $ & $    7.90_{ -0.15}^{+  0.20} $ & $  4.16_{ -0.13}^{+  0.06} $ &  4.40 \\
    B066-G128 &   -0.02 &  $    7.51_{ -0.63}^{+  0.45} $ & $    7.85_{ -0.15}^{+  0.15} $ & $  3.68_{ -0.72}^{+  0.24} $ &  4.20 \\
    B081-G142 &   -0.02 &  $    8.43_{ -0.53}^{+  0.23} $ & $    8.15_{ -0.15}^{+  0.15} $ & $  4.57_{ -0.29}^{+  0.14} $ &  5.10 \\
   B257D-D073 &   -0.02 &  $    7.98_{ -0.16}^{+  0.40} $ & $    7.90_{ -0.15}^{+  0.20} $ & $  4.11_{ -0.09}^{+  0.23} $ &  4.60 \\
    B318-G042 &   -0.40 &  $    7.78_{ -0.28}^{+  0.20} $ & $    7.85_{ -0.15}^{+  0.15} $ & $  4.01_{ -0.18}^{+  0.10} $ &  3.80 \\
    B321-G046 &    0.65 &  $    7.75_{ -0.15}^{+  0.03} $ & $    8.23_{ -0.15}^{+  0.10} $ & $  3.94_{ -0.07}^{+  0.02} $ &  4.20 \\
    B327-G053 &   -0.40 &  $    7.68_{ -0.24}^{+  0.26} $ & $    7.70_{ -0.10}^{+  0.15} $ & $  4.21_{ -0.14}^{+  0.15} $ &  4.50 \\
    B376-G309 &   -0.02 &  $    7.94_{ -0.29}^{+  0.36} $ & $    8.00_{ -0.15}^{+  0.15} $ & $  3.89_{ -0.18}^{+  0.21} $ &  4.10 \\
    B448-D035 &   -0.02 &  $    8.47_{ -0.27}^{+  0.08} $ & $    7.90_{ -0.15}^{+  0.20} $ & $  4.47_{ -0.16}^{+  0.05} $ &  4.10 \\
    B475-V128 &   -0.40 &  $    8.02_{ -0.35}^{+  0.06} $ & $    8.30_{ -0.20}^{+  0.20} $ & $  4.28_{ -0.19}^{+  0.04} $ &  4.70 \\
         V031 &   -0.70 &  $    8.50_{ -0.41}^{+  0.46} $ & $    8.45_{ -0.15}^{+  0.15} $ & $  4.14_{ -0.22}^{+  0.29} $ &  4.80 \\
   VDB0-B195D &   -0.02 &  $    7.78_{ -0.20}^{+  0.04} $ & $    7.40_{ -0.30}^{+  0.30} $ & $  4.96_{ -0.11}^{+  0.03} $ & 99.99 \\
    B083-G146 &   -0.40 &  $    8.88_{ -0.18}^{+  0.11} $ & $    8.70_{  0.00}^{+  1.44} $ & $  4.67_{ -0.11}^{+  0.06} $ &  4.70 \\
    B222-G277 &   -0.02 &  $    8.86_{ -0.06}^{+  0.05} $ & $    8.60_{  0.00}^{+  1.54} $ & $  4.59_{ -0.05}^{+  0.04} $ &  4.60 \\
    B347-G154 &   -0.40 &  $    8.92_{ -0.07}^{+  0.07} $ & $    8.80_{  0.00}^{+  1.34} $ & $  4.76_{ -0.04}^{+  0.04} $ &  4.70 \\
    B374-G306 &   -0.02 &  $    8.40_{ -0.26}^{+  0.17} $ & $    8.50_{  0.00}^{+  1.64} $ & $  4.05_{ -0.15}^{+  0.10} $ &  3.90 \\
         NB16 &   -0.02 &  $    9.08_{ -0.06}^{+  0.66} $ & $    8.70_{  0.00}^{+  1.44} $ & $  4.75_{ -0.05}^{+  0.59} $ &  4.80 \\
    B049-G112 &   -0.02 &  $    8.49_{ -0.11}^{+  0.21} $ & $    8.45_{ -0.20}^{+  0.20} $ & $  4.40_{ -0.05}^{+  0.15} $ &  4.50 \\
    B367-G292 &   -0.02 &  $    8.37_{ -0.05}^{+  0.06} $ & $    8.30_{ -0.20}^{+  0.20} $ & $  4.06_{ -0.02}^{+  0.03} $ &  4.30 \\
    B458-D049 &   -0.02 &  $    8.52_{ -0.14}^{+  0.16} $ & $    8.50_{ -0.20}^{+  0.20} $ & $  4.24_{ -0.07}^{+  0.11} $ &  4.10 \\
  B521-SK034A &   -0.02 &  $    7.81_{ -0.11}^{+  0.05} $ & $    8.60_{ -0.30}^{+  0.30} $ & $  3.72_{ -0.08}^{+  0.03} $ &  3.90 \\
         M039 &   -0.02 &  $    8.26_{ -0.31}^{+  0.43} $ & $    8.50_{ -0.20}^{+  0.20} $ & $  3.47_{ -0.17}^{+  0.26} $ &  3.80 \\
         M050 &   -0.02 &  $    8.15_{ -0.26}^{+  0.31} $ & $    8.75_{ -0.30}^{+  0.30} $ & $  3.56_{ -0.14}^{+  0.17} $ &  4.30 \\
    B315-G038 &   -0.40 &  $    7.86_{ -0.34}^{+  0.14} $ & $    8.00_{ -0.20}^{+  0.15} $ & $  4.60_{ -0.22}^{+  0.06} $ &  4.60 \\
    B319-G044 &   -0.40 &  $    7.78_{ -0.38}^{+  0.22} $ & $    8.00_{ -0.20}^{+  0.15} $ & $  3.94_{ -0.23}^{+  0.11} $ &  3.90 \\
    B342-G094 &   -0.40 &  $    8.00_{ -0.16}^{+  0.08} $ & $    8.20_{ -0.20}^{+  0.15} $ & $  3.87_{ -0.07}^{+  0.05} $ &  4.00 \\
    B368-G293 &   -0.02 &  $    7.56_{ -0.67}^{+  0.49} $ & $    7.80_{ -0.10}^{+  0.10} $ & $  3.61_{ -0.73}^{+  0.27} $ &  4.40 \\
    B292-G010 &   -1.82 &  $    9.24_{ -0.12}^{+  0.06} $ & $    9.80_{  0.00}^{+  0.34} $ & $  4.62_{ -0.12}^{+  0.02} $ & 99.99 \\
    B337-G068 &   -1.30 &  $    9.30_{ -0.04}^{+  0.13} $ & $    9.65_{  0.00}^{+  0.49} $ & $  4.75_{ -0.01}^{+  0.09} $ & 99.99 \\
    B350-G162 &   -1.52 &  $    9.30_{ -0.04}^{+  0.08} $ & $    9.75_{  0.00}^{+  0.39} $ & $  4.79_{ -0.01}^{+  0.06} $ & 99.99 \\

